Minimizing Polarization and Disagreement in the Friedkin-Johnsen Model with Unknown Innate Opinions

The bulk of the literature on opinion optimization in social networks adopts the Friedkin-Johnsen (FJ) opinion dynamics model, in which the innate opinions of all nodes are known: this is an unrealistic assumption. In this paper, we study opinion optimization under the FJ model without the full knowledge of innate opinions. Specifically, we borrow from the literature a series of objective functions, aimed at minimizing polarization and/or disagreement, and we tackle the budgeted optimization problem, where we can query the innate opinions of only a limited number of nodes. Given the complexity of our problem, we propose a framework based on three steps: (1) select the limited number of nodes we query, (2) reconstruct the innate opinions of all nodes based on those queried, and (3) optimize the objective function with the reconstructed opinions. For each step of the framework, we present and systematically evaluate several effective strategies. A key contribution of our work is a rigorous error propagation analysis that quantifies how reconstruction errors in innate opinions impact the quality of the final solutions. Our experiments on various synthetic and real-world datasets show that we can effectively minimize polarization and disagreement even if we have quite limited information about innate opinions.

==> Intro.tex <==
The rise of social media has substantially changed the way that people form their opinions~\cite{whiting13people}. Compared with the previous age, individuals are more easily affected by others' opinions, and consequently the public opinion tends to be driven to an extreme state~\cite{Bail18exposure}. In this situation, it is crucial to thoroughly analyze the dynamics of peoples' opinions and to develop an effective intervention approach to mitigate any perilous state of the public opinion such as polarization and disagreement~\cite{musco2018minimizing,cinus2023rebalancing,zhu2021minimizing}. 

There are many existing models that mathematically formulate the dynamics of opinions~\cite{rainer2002opinion}. Among them, the Friedkin--Johnsen (FJ) model has garnered much attention both in theory and in practice~\cite{friedkin1990social}. In the most general form of this model, we are given an edge-weighted directed social network, where each node corresponds to a user of a social platform and each directed edge $(i,j)$ indicates that user $i$ follows user $j$ or, in other words, that $j$ can influence $i$. The edge weight for $(i,j)$ quantifies how much $j$ exerts influence over $i$, e.g., the amount of contents produced by $j$ that is shared with $i$. In addition, each node has a parameter called an \emph{innate opinion}, which represents the degree of agreement of the node about the specific topic we are focusing on. 

The dynamics of expressed opinions evolve, based on the network structure and the innate opinions, in a discrete-time fashion: 
Initially the opinions of nodes are represented by their innate opinions. Then, at each time step, the opinion of each node is updated by averaging its innate opinion and the expressed opinions of its followees, weighted according to the edge weights. It is well known that the equilibrium state of opinions has an analytic from based on the Laplacian of the network and the innate opinions. To date, a variety of measures have been invented to quantify some characteristics of the equilibrium opinions. 
    
The seminal work of Musco et al.~\cite{musco2018minimizing} defined the measures of \emph{polarization} and \emph{disagreement} of the equilibrium opinions of the FJ model on undirected networks. 
The polarization is defined to be the deviation of the opinions of users from the average opinion, while the disagreement is defined to be the sum of weighted differences between neighboring opinions. 
Based on these, Musco et al.~\cite{musco2018minimizing} introduced the problem of minimizing the sum of polarization and disagreement by intervening the weights of edges, and designed a polynomial-time approximation scheme based on the convexity of the objective function. 

Very recently, Cinus et al.~\cite{cinus2023rebalancing} extended the above problem to general directed networks and reformulated it in the context of \emph{rebalancing social feed}. 
Specifically, the intervention is to rebalance the weights of out-going edges of each node, i.e., re-weight the relative importance of the accounts that the user follows, so as to calibrate the frequency with which the content produced by various accounts is shown to the user. Their approach, by re-balancing the weight of existing links, preserves the total engagement of each user in the social network.

However, existing algorithms for any problem of minimizing polarization and disagreement assume the full knowledge about the innate opinions of users; they require that information \emph{as input}. This assumption is quite strong, which rarely holds. Indeed, in practice, it may be quite costly and therefore impossible to acquire the innate opinions of users. For instance, consider the case where we analyze opinions of Twitter users about some political topic (e.g., COVID-19 vaccination and Brexit) in the Twitter follower--followee network. In this case, to obtain users' innate opinions, we have to conduct a large-scale survey or carefully analyze users' behaviors (e.g., tweets, retweets, and likes). Even if we do that, it is not necessarily sufficient. 

In this paper, to overcome the limitation, we initiate the problem of minimizing polarization and disagreement that does not assume the full knowledge of innate opinions. 
Our problem is built upon the aforementioned problems of Musco et al.~\cite{musco2018minimizing} and Cinus et al.~\cite{cinus2023rebalancing}, but 
relies solely on the assumption that we can query only a limited number of innate opinions among those in the entire network. 
In this challenging scenario, we are asked to minimize the sum of polarization and disagreement (or either of the two) defined over the unknown innate opinions. 

To address our problem, it seems crucial to effectively estimate the innate opinions of nodes that we did not query, based on those queried. To analyze its importance, we first quantify how the estimation error of innate opinions affects the final quality of solutions in terms of minimizing polarization and disagreement.  
Specifically, we upper bound the difference between the objective values achieved when we have the full knowledge of innate opinions and when we only have the estimated innate opinions, by the estimation error and the Lipschitz constants of the objective functions. 
Moreover, we examine the convexity and non-convexity of the objective functions, which characterize the solvability of problems. 


From an algorithmic perspective, we present several strategies for each of (i) selection of nodes that we will query the innate opinions and (ii) estimation of innate opinions of nodes that we did not query, based on those we queried. 
As for Step (i), we consider several node selection rules for Step (i), based on some centrality measures, including the degree centrality, closeness centrality, and PageRank. 
\atsushi{Our selection of centrality measures is based on...}
As for Step (ii), we employ three strategies based on label propagation~\cite{zhu2002learning}, graph neural networks~\cite{}, and graph signal processing~\cite{lorenzo2018sampling}. 
Our selection of opinion estimation algorithms is based on the fact that in real-world networks, the innate opinions present the strong \emph{homophily}, meaning that the innate opinions of neighbors tend to be similar. 

We conduct thorough computational experiments using various synthetic and real-world datasets, and empirically evaluate the performance of algorithms. 
Our main finding is that we can minimize the sum of polarization and disagreement (or either of the two) even if we have a quite limited information about the innate opinions, using appropriate combinations of node selection rules and opinion estimation algorithms. 
Moreover, we confirm the validity of the above discussion about the effect of the estimation error in the final quality of solutions. 

Our contribution can be summarized as follows: 
\begin{itemize}
\leftskip=-15pt
\item We initiate the problem of minimizing polarization and disagreement without assuming the full knowledge of innate opinions. 
\item 
\item 
\item 
\end{itemize}



==> Related.tex <==
The study of social media through the lenses of bias, polarization, and echo chambers is currently an intensive and controversial area of research~\cite{falkenberg2022growing,nyhan2023like,avalle2024persistent,allcott2024effects}.

\spara{Modeling Polarization in Social Media.}
From a theoretical computer science perspective, significant effort has been invested in characterizing polarization using the Friedkin–Johnsen (FJ) opinion-dynamics model~\cite{friedkin1990social,bindel2015bad}.
In this model, social media users are depicted as nodes within a network, while their connections are represented as edges. The model operates through an iterative process where users adjust their opinions by taking a weighted average of their own views and those of their connected peers. 
Due to its linear algebraic nature, the model has inspired several discrete and continuous optimization problems involving susceptibility~\cite{abebe2021opinion,marumo2021projected}, stubbornness~\cite{xu2022effects}, exposure timelines~\cite{zhou2024modeling}, and adversarial attacks~\cite{tu2023adversaries}.

\spara{Minimizing Polarization and Disagreement.}
Among the various optimization problems in FJ models, minimizing polarization and disagreement plays a pivotal role. 
First introduced by \citet{musco2018minimizing}, the problem aims to reduce polarization and disagreement simultaneously, which they proved to be a matrix-convex objective, in undirected social graphs by continuously changing the network weights. Different modeling and intervention strategies have been explored~\cite{abebe2021opinion,zhu2021minimizing,zhou2024modeling}.
Among all, recently, \citet{cinus2023rebalancing} introduced the problem of minimizing polarization and disagreement in a probabilistic directed graph by only adjusting weights associated with pre-existing edges. Although this approach is the closest to ours in terms of generality in optimization problems and solving strategies, it assumes that all inner opinions are known in advance, which may not always be realistic.

\spara{Evaluation of Polarization and Disagreement.}
In the continuous setting, \citet{chen2018quantifying} simultaneously characterized how to evaluate and optimize conflict measures related to the FJ model in social networks, investigating optimization potential across all sets of prior opinions in average- and worst-case scenarios using gradient descent. \citet{xu2021fast} focused exclusively on the efficient evaluation of these quantities using Laplacian solvers.

To the best of our knowledge, \citet{neumann2024sublinear} is the first to extend this problem to the setting of unknown opinions. Their estimations can be done efficiently in sublinear time with respect to the number of nodes. 
However, when estimating a single expressed opinion, their algorithm requires an undirected graph as input, and a number of oracle calls to retrieve unknown innate opinions. 
Although this number is sublinear for recovering one opinion, extending the algorithm to recover the whole set of nodes could, in the worst-case scenario, exceed a possible small budget constraint.
\federico{atsushi, please make a pass. I'm still not convinced by my comment. I think there is a way to use Stefan's results in our case. If you agree, Check also Table 1 in their paper: the error in polarization and disagreement is linear in n; does it mean that they get a larger error when minimizing these objectives compared to our constant errors?}




Our contribution differs from previous works in that it combines the optimization of FJ quantities (polarization, disagreement, and their sum in directed and undirected cases) and opinion recovery under budget constraints, analyzed in a worst-case scenario. We also test different heuristic strategies to solve these problems.


==> tikzlibrarybayesnet.code.tex <==

\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
\tikzstyle{obs} = [latent,fill=gray!25]
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
\tikzstyle{det} = [latent, diamond]

\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %


\newcommand{\factoredge}[4][]{ %
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->, >={triangle 45}, #1] (\y) ; %
    } ;
  } ;
}

\newcommand{\edge}[3][]{ %
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->, >={triangle 45}, #1] (\y) ;%
    } ;
  } ;
}

\newcommand{\factor}[5][]{ %
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  \factoredge {#4} {#2-alias} {#5} ; %
}

\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

\newcommand{\vgate}[6]{ %
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  \draw [-, dashed] (#1.north) -- (#1.south); %
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

\newcommand{\hgate}[6]{ %
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  \draw [-, dashed] (#1.west) -- (#1.east); %
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

